Classicality without local discriminability: decoupling entanglement and complementarity

An operational probabilistic theory where all systems are classical, and all pure states of composite systems are entangled, is constructed. The theory is endowed with a rule for composing an arbitrary number of systems, and with a nontrivial set of transformations. Hence, we demonstrate that the presence of entanglement is independent of the existence of incompatible measurements. We then study a variety of phenomena occurring in the theory -- some of them contradicting both Classical and Quantum Theories -- including: cloning, entanglement swapping, dense coding, additivity of classical capacities, non-monogamous entanglement, hypersignaling. We also prove the existence, in the theory, of a universal processor. The theory is causal and satisfies the no-restriction hypothesis. At the same time, it violates a number of information-theoretic principles enjoyed by Quantum Theory, most notably: local discriminability, purity of parallel composition of states, and purification. Moreover, we introduce an exhaustive procedure to construct generic operational probabilistic theories, and a sufficient set of conditions to verify their consistency. In addition, we prove a characterisation theorem for the parallel composition rules of arbitrary theories, and specialise it to the case of bilocal-tomographic theories. We conclude pointing out some open problems. In particular, on the basis of the fact that every separable state of the theory is a statistical mixture of entangled states, we formulate a no-go conjecture for the existence of a local-realistic ontological model.

==> myqcircuit.tex <==
%    Q-circuit version 1.2
%    Copyright (C) 2004  Steve Flammia & Bryan Eastin, 4/23/06
%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.
%
%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.
%
%    You should have received a copy of the GNU General Public License
%    along with this program; if not, write to the Free Software
%    Foundation, Inc., 59 Temple Place, Suite 330, Boston, MA  02111-1307  USA

\usepackage[matrix,frame,arrow]{xy}
\usepackage{amsmath}
\newcommand{\bra}[1]{\left\langle{#1}\right\vert}
\newcommand{\ket}[1]{\left\vert{#1}\right\rangle}
    % Defines Dirac notation.
\newcommand{\qw}[1][-1]{\ar @{-} [0,#1]}
    % Defines a wire that connects horizontally.  By default it connects to the object on the left of the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\qwx}[1][-1]{\ar @{-} [#1,0]}
    % Defines a wire that connects vertically.  By default it connects to the object above the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\cw}[1][-1]{\ar @{=} [0,#1]}
    % Defines a classical wire that connects horizontally.  By default it connects to the object on the left of the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\cwx}[1][-1]{\ar @{=} [#1,0]}
    % Defines a classical wire that connects vertically.  By default it connects to the object above the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\gate}[1]{*{\xy *+<.6em>{#1};p\save+LU;+RU **\dir{-}\restore\save+RU;+RD **\dir{-}\restore\save+RD;+LD **\dir{-}\restore\POS+LD;+LU **\dir{-}\endxy} \qw}
    % Boxes the argument, making a gate.
\newcommand{\meter}{\gate{\xy *!<0em,1.1em>h\cir<1.1em>{ur_dr},!U-<0em,.4em>;p+<.5em,.9em> **h\dir{-} \POS <-.6em,.4em> *{},<.6em,-.4em> *{} \endxy}}
    % Inserts a measurement meter.
\newcommand{\measure}[1]{*+[F-:<.9em>]{#1} \qw}
    % Inserts a measurement bubble with user defined text.
\newcommand{\measuretab}[1]{*{\xy *+<.6em>{#1};p\save+LU;+RU **\dir{-}\restore\save+RU;+RD **\dir{-}\restore\save+RD;+LD **\dir{-}\restore\save+LD;+LC-<.5em,0em> **\dir{-} \restore\POS+LU;+LC-<.5em,0em> **\dir{-} \endxy} \qw}
    % Inserts a measurement tab with user defined text.
\newcommand{\measureD}[1]{*{\xy*+=+<.5em>{\vphantom{\rule{0em}{.1em}#1}}*\cir{r_l};p\save*!R{#1} \restore\save+UC;+UC-<.5em,0em>*!R{\hphantom{#1}}+L **\dir{-} \restore\save+DC;+DC-<.5em,0em>*!R{\hphantom{#1}}+L **\dir{-} \restore\POS+UC-<.5em,0em>*!R{\hphantom{#1}}+L;+DC-<.5em,0em>*!R{\hphantom{#1}}+L **\dir{-} \endxy} \qw}
    % Inserts a D-shaped measurement gate with user defined text.
\newcommand{\multimeasure}[2]{*+<1em,.9em>{\hphantom{#2}} \qw \POS[0,0].[#1,0];p !C *{#2},p \drop\frm<.9em>{-}}
    % Draws a multiple qubit measurement bubble starting at the current position and spanning #1 additional gates below.
    % #2 gives the label for the gate.
    % You must use an argument of the same width as #2 in \ghost for the wires to connect properly on the lower lines.
\newcommand{\multimeasureD}[2]{*+<1em,.9em>{\hphantom{#2}}\save[0,0].[#1,0];p\save !C *{#2},p+LU+<0em,0em>;+RU+<-.8em,0em> **\dir{-}\restore\save +LD;+LU **\dir{-}\restore\save +LD;+RD-<.8em,0em> **\dir{-} \restore\save +RD+<0em,.8em>;+RU-<0em,.8em> **\dir{-} \restore \POS !UR*!UR{\cir<.9em>{r_d}};!DR*!DR{\cir<.9em>{d_l}}\restore \qw}
    % Draws a multiple qubit D-shaped measurement gate starting at the current position and spanning #1 additional gates below.
    % #2 gives the label for the gate.
    % You must use an argument of the same width as #2 in \ghost for the wires to connect properly on the lower lines.
\newcommand{\control}{*!<0em,.025em>-=-{\bullet}}
    % Inserts an unconnected control.
\newcommand{\controlo}{*-<.21em,.21em>{\xy *=<.59em>!<0em,-.02em>[o][F]{}\POS!C\endxy}}
    % Inserts a unconnected control-on-0.
\newcommand{\ctrl}[1]{\control \qwx[#1] \qw}
    % Inserts a control and connects it to the object #1 wires below.
\newcommand{\ctrlo}[1]{\controlo \qwx[#1] \qw}
    % Inserts a control-on-0 and connects it to the object #1 wires below.
\newcommand{\targ}{*!<0em,.019em>=<.79em,.68em>{\xy {<0em,0em>*{} \ar @{ - } +<.4em,0em> \ar @{ - } -<.4em,0em> \ar @{ - } +<0em,.36em> \ar @{ - } -<0em,.36em>},<0em,-.019em>*+<.8em>\frm{o}\endxy} \qw}
    % Inserts a CNOT target.
\newcommand{\qswap}{*=<0em>{\times} \qw}
    % Inserts half a swap gate. 
    % Must be connected to the other swap with \qwx.
\newcommand{\multigate}[2]{*+<1em,.9em>{\hphantom{#2}} \qw \POS[0,0].[#1,0];p !C *{#2},p \save+LU;+RU **\dir{-}\restore\save+RU;+RD **\dir{-}\restore\save+RD;+LD **\dir{-}\restore\save+LD;+LU **\dir{-}\restore}
    % Draws a multiple qubit gate starting at the current position and spanning #1 additional gates below.
    % #2 gives the label for the gate.
    % You must use an argument of the same width as #2 in \ghost for the wires to connect properly on the lower lines.
\newcommand{\ghost}[1]{*+<1em,.9em>{\hphantom{#1}} \qw}
    % Leaves space for \multigate on wires other than the one on which \multigate appears.  Without this command wires will cross your gate.
    % #1 should match the second argument in the corresponding \multigate. 
\newcommand{\push}[1]{*{#1}}
    % Inserts #1, overriding the default that causes entries to have zero size.  This command takes the place of a gate.
    % Like a gate, it must precede any wire commands.
    % \push is useful for forcing columns apart.
    % NOTE: It might be useful to know that a gate is about 1.3 times the height of its contents.  I.e. \gate{M} is 1.3em tall.
    % WARNING: \push must appear before any wire commands and may not appear in an entry with a gate or label.
\newcommand{\gategroup}[6]{\POS"#1,#2"."#3,#2"."#1,#4"."#3,#4"!C*+<#5>\frm{#6}}
    % Constructs a box or bracket enclosing the s % \begin{equation*}
%   \begin{aligned}
%     \Qcircuit @C=1em @R=.7em @! R {& \qw \poloFantasmaCn \sA & \multigate{1} 
% {\Transformation{A}_i \otimes \Transformation{B}_j} & \qw
%       \poloFantasmaCn \sB &\qw\\
%       & \qw \poloFantasmaCn \sC & \ghost {\Transformation{A}_i\otimes 
% \Transformation{B}_j} & \qw \poloFantasmaCn \sD &\qw}
%   \end{aligned}=
%   \begin{aligned}
%     \Qcircuit @C=1em @R=.7em @! R {& \qw \poloFantasmaCn \sA & \gate 
% {\Transformation{A}_i} & \qw \poloFantasmaCn \sB
%     &\qw\\ & \qw \poloFantasmaCn \sC & \gate{\Transformation{B}_j} & \qw 
% \poloFantasmaCn \sD &\qw}
%   \end{aligned}
% \end{equation*}quare block spanning rows #1-#3 and columns=#2-#4.
    % The block is given a margin #5/2, so #5 should be a valid length.
    % #6 can take the following arguments -- or . or _\} or ^\} or \{ or \} or _) or ^) or ( or ) where the first two options yield dashed and
    % dotted boxes respectively, and the last eight options yield bottom, top, left, and right braces of the curly or normal variety.
    % \gategroup can appear at the end of any gate entry, but it's good form to pick one of the corner gates.
    % BUG: \gategroup uses the four corner gates to determine the size of the bounding box.  Other gates may stick out of that box.  See \prop. 
\newcommand{\rstick}[1]{*!L!<-.5em,0em>=<0em>{#1}}
    % Centers the left side of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\lstick}[1]{*!R!<.5em,0em>=<0em>{#1}}
    % Centers the right side of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\ustick}[1]{*!D!<0em,-.5em>=<0em>{#1}}
    % Centers the bottom of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\dstick}[1]{*!U!<0em,.5em>=<0em>{#1}}
    % Centers the top of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\Qcircuit}[1][0em]{\xymatrix @*=<#1>}
    % Defines \Qcircuit as an \xymatrix with entries of default size 0em.  The optional argument, #1, is for use with clusters, and allows you
    % to fix the size of the nodes.  I would not advise using it with normal circuits.
\newcommand{\node}[2][]{{\begin{array}{c} \ _{#1}\  \\ {#2} \\ \ \end{array}}\drop\frm{o} }
    % When Qcircuit has been passed the optional argument for cluster states, this command produces a round node of the size specified in that
    % argument.  The optional argument #2 specifies the contents of a node, while optional argument #1 is a secondary label.  
\newcommand{\link}[2]{\ar @{-} [#1,#2]}
    % Draws a wire or connecting line to the element #1 rows down and #2 columns forward.
\newcommand{\pureghost}[1]{*+<1em,.9em>{\hphantom{#1}}}
    % Same as \ghost except it omits the wire leading to the left. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\multiprepareC}[2]{*+<1em,.9em>{\hphantom{#2}}\save[0,0].[#1,0];p\save !C
  *{#2},p+RU+<0em,0em>;+LU+<+.8em,0em> **\dir{-}\restore\save +RD;+RU **\dir{-}\restore\save
  +RD;+LD+<.8em,0em> **\dir{-} \restore\save +LD+<0em,.8em>;+LU-<0em,.8em> **\dir{-} \restore \POS
  !UL*!UL{\cir<.9em>{u_r}};!DL*!DL{\cir<.9em>{l_u}}\restore}
   % Draws a multiple qubit reverse-D-shaped preparation gate starting at the current position and spanning #1 additional gates below.
   % #2 gives the label for the gate.
   % You must use an argument of the same width as #2 in \pureghost for the wires to connect properly on
% the lower lines.
   % Inserts a reverse-D-shaped preparation gate with user defined text.
\newcommand{\prepareC}[1]{*{\xy*+=+<.5em>{\vphantom{#1\rule{0em}{.1em}}}*\cir{l^r};p\save*!L{#1} \restore\save+UC;+UC+<.5em,0em>*!L{\hphantom{#1}}+R **\dir{-} \restore\save+DC;+DC+<.5em,0em>*!L{\hphantom{#1}}+R **\dir{-} \restore\POS+UC+<.5em,0em>*!L{\hphantom{#1}}+R;+DC+<.5em,0em>*!L{\hphantom{#1}}+R **\dir{-} \endxy}}

\newcommand{\poloFantasmaCn}[1]{{{}^{#1}_{\phantom{#1}}}}


% Aggiunte di Franco


==> preamble.tex <==
\usepackage{url}
\def\UrlBreaks{\do\/\do-}
\usepackage{breakurl}
\usepackage{epsfig,amssymb,amsmath,mathrsfs,color}
\RequirePackage[colorlinks=true,linkcolor=blue,urlcolor=blue,citecolor=blue,linktocpage,breaklinks]{hyperref}
\usepackage{comment}
\usepackage{amsthm}
\def\bh{\mathbf{h}}
\def\<{\langle}\def\>{\rangle}
\def\rank{\operatorname{rank}}\def\Sym{\operatorname{Sym}}
\def\dist{\operatorname{dist}}\def\supp{\operatorname{Supp}}
\def\n#1{\|#1\|}
\def\sH{\mathcal{H}}
\def\Cmplx{\mathbb{C}}\def\Reals{\mathbb{R}}\def\N{\mathbb{N}}\def\Z{\mathbb{Z}}\def\M{\mathbb{M}}
\usepackage{hyperref}
\usepackage{enumerate}
\usepackage[shortlabels]{enumitem} %inline

\DeclareSymbolFont{sfletters}{OML}{cmbrm}{m}{it}
\DeclareMathSymbol{\srho}{\mathord}{sfletters}{"1A}
\DeclareMathSymbol{\svarrho}{\mathord}{sfletters}{"25}

\include{myqcircuit}

\newcommand\bibit{bibit}
\newcommand{\rbra}[1]{({#1}\vert}
\newcommand{\rket}[1]{\vert{#1})}
\newcommand{\arbra}[1]{\left({#1}\right\vert}
\newcommand{\arket}[1]{\left\vert{#1}\right)}
\newcommand{\rbraket}[2]{( #1 \vphantom{#2} | #2 \vphantom{#1} )}
\newcommand{\arbraket}[2]{\left( #1 \vphantom{#2} \right|\left. #2 \vphantom{#1} \right)}

\theoremstyle{plain}
%\theoremstyle{remark}
\newtheorem*{definition*}{Definition}
\newtheorem{definition}{Definition}
\newtheorem{postulate}{Postulate}
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{proposition*}{Proposition}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem*{question*}{Question}
\newtheorem{question}{Question}
\newtheorem*{problem*}{Problem}
\newtheorem{problem}{Problem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{lemma}{Lemma}
\newtheorem*{example*}{Example}
\newtheorem{example}{Example}
\newtheorem{property}{Property}
\newtheorem*{property*}{Property}
\newtheorem*{remark*}{Remark}
\newtheorem{remark}{Remark}
\newtheorem*{proof*}{Proof}

\usepackage{graphicx}
\usepackage{epsfig}
\usepackage[matrix,frame,arrow]{xypic}
\vfuzz2pt
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage{comment}
%\usepackage[font=small,labelfont=bf,
%   justification=justified,
%   format=plain]{caption}
%\usepackage[font=small,labelfont=bf,
%justification=justified,
%format=plain]{subcaption}
%\captionsetup[subfigure]{justification=justified,labelformat=simple}%,labelsep=colon}
%\renewcommand{\thesubfigure}{(\alph{subfigure})}

\renewcommand{\v}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\gv}[1]{\ensuremath{\mbox{\boldmath$ #1 $}}} 
\newcommand{\braket}[2]{\left< #1 \vphantom{#2} | #2 \vphantom{#1} \right>}
%\newtheorem{lemma}{Lemma} \newtheorem{remark}{Remark} 
%\newtheorem{proposition}{Proposition}
%\newtheorem{example}{Example}
%\newtheorem*{example*}{Example}
%\newtheorem{corollary}{Corollary} \newtheorem{theorem}{Theorem}
 %\newtheorem{definition}{Definition}
\def\bvec#1{\mathbf{#1}}
\def\bk{\bvec k}
\def\bh{\bvec h}
\def\bik{{\bvec  k'}}
\def\bn{\bvec n} 
\def\bl{\bvec l} 
\def\bm{\bvec m}
\def\spc #1{{\mathsf #1}}
\def\Proof{\medskip\par\noindent{\bf Proof.  }}
\def\qed{$\,\blacksquare$\par} \def\>{\rangle} \def\<{\langle}
\def\kk{\>\! \>}\def\bb{\<\!\<} \def\map#1{\mathscr #1}
\def\lntrnsfrm#1{\mathrm #1} \def\sys#1{\mathrm{#1}} \def\rA{{\sys
    A}}\def\rB{{\sys B}}\def\rC{{\sys C}}\def\rD{{\sys D}}
\def\rE{{\sys E}} \def\rF{{\sys F}} \def\rG{{\sys G}} \def\rI{{\sys
    I}}\def\rc{{\sys c}} \def\rR{{\sys R}} \def\rS{{\sys
    S}}\def\rX{\sys X}\def\rY{\sys Y}\def\rZ{\sys Z}
\def\samp#1{\mathrm{#1}} \def\cX{{\samp X}} \def\cY{{\samp
    Y}}\def\cZ{{\samp Z}} \def\sH{{\spc H}} \def\sI{{\spc I}}
\def\tA{\map A}\def\tB{\map B}\def\tC{\map C}\def\tD{\map D}
\def\tS{\map S}\def\tG{\map G}\def\tL{\map L}\def\tK{\map K}
\def\tI{\map I}\def\tT{\map T}\def\tU{\map U} \def\tV{\map V}
\def\tW{\map W}\def\tM{\map M}\def\tX{\map X} \def\tY{\map
  Y}\def\tZ{\map Z}\def\tF{\map F}\def\tO{\map O}\def\tE{\map E}
\def\tJ{\map J}\def\tR{\map R}\def\tP{\map P }\def\tS{\map S}
\def\tT{\map T} \def\Cntset{\mathsf{Eff}} \def\grp#1{{\mathbf{#1}}}
\def\Span{\mathsf{Span}} \def\Stset{\mathsf{St}} \def\Trnset{{\mathsf
    T}} \def\K#1{\left|#1\right)\!}
\def\aff{\mathsf{Aff}}\def\con{\mathsf K}\def\det{\mathsf N}
\def\B#1{\left(#1\right|}
%  \def\SC#1#2{\left({#1}\right|\left.\!{#2}\right)\!}  
\def\Tr{{\rm Tr}} \def\Eta{\rm{H}} \def\Reals{{\mathbb R}}
\def\ch{\ensuremath{\mathfrak{C}}} \def\cu{\ensuremath{\mathsf C}}
\newcommand\remind[1]{\marginpar{\baselineskip=6pt$\blacktriangleright$
    \raggedright{\tiny #1 }}}
\newcommand\marginlabel[1]{\marginpar{#1}}

\usepackage[usenames,dvipsnames]{xcolor}
\def\nota#1{\textcolor{BurntOrange}{\textbf{#1}}}
\usepackage{soul}

\newcommand{\ExtSt}[1]{\ensuremath{\mathsf{ExtSt}(\mathrm{#1})}}
\newcommand{\ExtStZ}[1]{\ensuremath{\mathsf{ExtSt}_0(\mathrm{#1})}}
\newcommand{\s}[1]{\ustick{\scriptstyle{\sys{#1}}}}
\newcommand{\Sys}[1]{\ensuremath{\mathsf{Sys(\mathrm{#1})}}}
\newcommand{\Ob}[1]{\ensuremath{\mathsf{Ob(\mathrm{#1})}}}
\newcommand{\syst}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\D}[1]{\ensuremath{D_\syst{#1}}}
\newcommand{\St}[1]{\ensuremath{\mathsf{St(\mathrm{#1})}}}
\newcommand{\StC}[1]{\ensuremath{\mathsf{St_+(\mathrm{#1})}}}
\newcommand{\StN}[1]{\ensuremath{\mathsf{St_1(\mathrm{#1})}}}
\newcommand{\StR}[1]{\ensuremath{\mathsf{St}_{\mathbb{R}}(\mathrm{#1})}}
\newcommand{\C}[1]{\ensuremath{\mathsf{S(\mathrm{#1})}}}
\newcommand{\PurSt}[1]{\ensuremath{\mathsf{PurSt(\mathrm{#1})}}}
\newcommand{\PurRef}[2]{\ensuremath{\mathsf{PurRef}_{#1}(\mathrm{#2})}}
\newcommand{\PurRefA}[1]{\ensuremath{\mathsf{PurRef}(\mathrm{#1})}}
\newcommand{\PurRefbar}[1]{\ensuremath{\overline{\mathsf{PurRef}}(\mathrm{#1})}}
\newcommand{\PS}[1]{\ensuremath{\mathsf{PrSt(\mathrm{#1})}}}
\newcommand{\ConvH}[1]{\ensuremath{\mathsf{ConvH(#1)}}}
\newcommand{\Eff}[1]{\ensuremath{\mathsf{Eff(\mathrm{#1})}}}
\newcommand{\EffR}[1]{\ensuremath{\mathsf{Eff}_{\mathbb{R}}(\mathrm{#1})}}
\newcommand{\EffC}[1]{\ensuremath{\mathsf{Eff_+(\mathrm{#1})}}}
\newcommand{\EffN}[1]{\ensuremath{\mathsf{Eff_1(\mathrm{#1})}}}
\newcommand{\E}[1]{\ensuremath{\mathsf{E(\mathrm{#1})}}}
\newcommand{\T}[1]{\ensuremath{\mathscr{#1}}}
\newcommand{\Transf}[2]{\ensuremath{\mathsf{Transf(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\TransfR}[2]{\ensuremath{\mathsf{Transf_{\mathbb{R}}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\TransfN}[2]{\ensuremath{\mathsf{Transf_{1}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\TransfC}[2]{\ensuremath{\mathsf{Transf_{+}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\transf}[1]{\ensuremath{\mathsf{Transf(\mathrm{#1})}}}
\newcommand{\Mor}[2]{\ensuremath{\mathsf{Mor(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\mor}[1]{\ensuremath{\mathsf{Mor(\mathrm{#1})}}}
\newcommand{\TransfA}[1]{\ensuremath{\mathsf{Transf(\mathrm{#1})}}}
\newcommand{\RevTransfA}[1]{\ensuremath{\mathsf{RevTransf(\mathrm{#1})}}}
\newcommand{\RevTransf}[2]{\ensuremath{\mathsf{RevTransf(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\LocTransf}[2]{\ensuremath{\mathsf{LocTransf(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\LocTransfA}[1]{\ensuremath{\mathsf{LocTransf(\mathrm{#1})}}}
\newcommand{\TestC}[4]{\ensuremath{\mathsf{#1}_{\mathsf{#2}}^{\mathrm{#3}\!\to\!\mathrm{#4}}}}
\newcommand{\TestAB}[2]{\ensuremath{\mathsf{Test(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\Test}[2]{\ensuremath{\mathsf{#1_{\mathsf{#2}}}}}
\newcommand{\TestA}[1]{\ensuremath{\mathsf{Test(\mathrm{#1})}}}
\newcommand{\InstrC}[4]{\ensuremath{\mathsf{#1}_{\mathsf{#2}}^{\mathrm{#3}\!\to\!\mathrm{#4}}}}
\newcommand{\InstrAB}[2]{\ensuremath{\mathsf{Instr(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\InstrABR}[2]{\ensuremath{\mathsf{Instr_{\mathbb{R}}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\Instr}[2]{\ensuremath{\mathsf{#1_{\mathsf{#2}}}}}
\newcommand{\InstrA}[1]{\ensuremath{\mathsf{Instr(\mathrm{#1})}}}
\newcommand{\Event}[2]{\ensuremath{\mathsf{Event(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\EventA}[1]{\ensuremath{\mathsf{Event(\mathrm{#1})}}}
\newcommand{\Out}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\Refi}[1]{\ensuremath{\mathsf{Ref}(\mathscr{#1})}}
\newcommand{\ConvRef}[1]{\ensuremath{\mathsf{ConvRef(\mathscr{#1})}}}

\usepackage{tikz}
\input{tikzit.sty}
\input{style.tikzstyles}
\usepackage{stmaryrd}
\usepackage{xpatch}

\makeatletter
\patchcmd{\@ssect@ltx}
{\addcontentsline{toc}{#1}{\protect\numberline{}#8}}
{}
{}
{}
\makeatother

\makeatletter
\def\@bibdataout@aps{%
	\immediate\write\@bibdataout{%
		@CONTROL{%
			apsrev41Control%
			\longbibliography@sw{%
				,author="08",editor="1",pages="1",title="0",year="1"%
			}{%
				,author="08",editor="1",pages="1",title="",year="1"%
			}%
		}%
	}%
	\if@filesw \immediate \write \@auxout {\string \citation {apsrev41Control}}\fi 
}
\makeatother
